The landscape of symmetry enhancement in tight-binding models

Band structures are ubiquitous in condensed matter physics and their symmetries constrain possible degeneracies, topology and response functions across a broad range of different systems. Here we address the question: given a parent crystal, what is the symmetry of hopping models on that lattice at a given shell number? We find that the parent structure does not, in general, determine the symmetry of the tight-binding model. Instead, the symmetry is dependent on the hopping range. The key to symmetry breakdown on the lattice is the existence of different {\it bond equivalence classes} whose number is related to group-subgroup indices for a broad classes of cases. We find all bond equivalence classes for $s$-wave hopping out to 20th neighbor across the different space groups and Wyckoff positions and the symmetries of the associated tight-binding models. These observations naturally lead to the definition of a {\it bond complex} $-$ the possible classes of networks of bonds to which symmetries may be enhanced from a given parent structure.

==> subfigure_code.tex <==
   \begin{figure*}
        \centering
        \begin{subfigure}[b]{0.325\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/p4_shell_k1.pdf}
            \caption[]{Shell $1$: $123(1c)$}
            %{{ Shell 1}}    
            \label{fig:s1}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.325\textwidth}  
            \centering 
            \includegraphics[width=\textwidth]{Figures/p4_shell_k2.pdf}
            \caption[]{Shell $2$: $123(1c)$}
            %\caption[]%
            %{{ Shell 2}}    
            \label{fig:s2}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.325\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{Figures/p4_shell_k3.pdf}
            \caption[]{Shell $3$: $125(2c)$}
            %\caption[]%
            %{{ Shell 3}}    
            \label{fig:s3}
        \end{subfigure}
          % \vskip\baselineskip	 
        \begin{subfigure}[b]{0.325\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/p4_shell_k4.pdf}
            \caption[]{Shell $4$: $123(2f)$}
            %\caption[Network2]%
            %{{Shell 4}}    
            \label{fig:s4}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.325\textwidth}  
            \centering 
            \includegraphics[width=\textwidth]{Figures/p4_shell_k5.pdf}
            \caption[]{Shell $5$: $123(2f)$}
           % \caption[]%
           % {{ Shell 5}}    
            \label{fig:s5}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.325\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{Figures/p4_shell_k6.pdf}
            \caption[]{Shell $6$: $123(1c)$}
           % \caption[]%
           % {{ Shell 6}}    
            \label{fig:s6}
        \end{subfigure}
          % \vskip\baselineskip	 

        \begin{subfigure}[b]{0.325\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/p4_shell_k7.pdf}
            \caption[]{Shell $7$: $127(2d)$}
           % \caption[Network2]%
           % {{ Shell 7}}    
            \label{fig:s7}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.325\textwidth}  
            \centering 
            \includegraphics[width=\textwidth]{Figures/p4_shell_k8.pdf}
            \caption[]{Shell $8$: $125(2c)$}
            %\caption[]%
           % {{ Shell 8}}    
            \label{fig:s8}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.325\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{Figures/p4_shell_k9.pdf}
            \caption[]{Shell $9$: $127(2d)$}
           % \caption[]%
           % {{ Shell 9}}    
            \label{fig:s9}
        \end{subfigure}
        %   \vskip\baselineskip	 

        \begin{subfigure}[b]{0.325\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/p4_shell_k10.pdf}
            \caption[]{Shell $10$: $83(1c)$}
           % \caption[Network2]%
           % {{ Shell 10}}    
            \label{fig:s10}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.325\textwidth}  
            \centering 
            \includegraphics[width=\textwidth]{Figures/p4_shell_k11.pdf}
            \caption[]{Shell $11$: $123(2f)$}
           % \caption[]%
           % {{ Shell 11}}    
            \label{fig:s11}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.325\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{Figures/p4_shell_k12.pdf}
            \caption[]{Shell $12$: $85(2a)$}
           % \caption[]%
           % {{ Shell 12}}    
            \label{fig:s12}
        \end{subfigure}
           \vskip\baselineskip	 
\caption[]{Band structures for tight-binding models at a given shell number for parent space group P4 and Wyckoff position 2c} 
\label{fig:bands}
\end{figure*}
